Sustained Kozai-Lidov oscillations in misaligned circumstellar gas disks

A disk around one component of a binary star system with sufficiently high inclination can undergo Kozai-Lidov (KL) oscillations during which the disk inclination and disk eccentricity are exchanged. Previous studies show that without a source of accretion, KL unstable disks exhibit damped oscillations, due to viscous dissipation, that leave the disk stable near or below the critical inclination for KL oscillations. With three-dimensional hydrodynamical simulations we show that a highly misaligned circumbinary disk that flows onto the binary components forms highly inclined circumstellar disks around each component. We show that a continuous infall of highly inclined material allows the KL oscillations to continue. The KL disk oscillations produce shocks and eccentricity growth in the circumstellar disks that affect the conditions for planet formation.

==> RESPONSE.tex <==
Reviewer's Comments:

The authors present a study of Kozai-Lidov oscillations induced in circum-individual discs in a binary where the orbital plane of the two stars is misaligned with respect to the plane of the outer disc. They demonstrate an interesting point, which is that Kozai-Lidov oscillations can be sustained in such discs by the infall from the outer disc. Overall the paper is well written and the result is interesting, and I am happy to recommend it for publication in ApJ Letters after some revisions. 

Major comments:

My only major comment concerns speculative claims about gravitational instability and planet formation. Conclusions about fragmentation seem hardly justified using simulations with a disk mass ratio of 10^-3. This is not demonstrated in the paper, so should be toned down both in the paper and in the abstract. Namely:

- in the discussion "Shocks may trigger..." needs to be tempered, e.g. by adding "in sufficiently massive discs". The authors should add a few sentences discussing how using a more massive outer disc might change some of the effects discussed. A outer disc that is sufficiently massive to be gravitationally unstable will supply an additional torque on the binary that may strongly affect the misalignment evolution, as the authors are well aware.

RESPONSE: We have made clear that sufficiently massive discs will trigger the gravitational instability. We have also added a paragraph in the discussion discussing the effects of a massive circumbinary disc will have on the binary and the alignment evolution. 

- truncate the abstract at "affect the conditions for planet formation". Speculation about fragmentation could be made in the discussion section but it is just speculation, so the abstract is not the place for it.

RESPONSE: We have truncated the abstract and added the information on fragmentation to the discussion section. 

- last sentence of the abstract, "strong shocks"->"shocks", since the strength of the shock is affected by the hack to increase the resolution in the inner disc. Should also clarify that you refer to the "shocks and eccentricity in the [circumstellar] discs"

RESPONSE: We have clarified (in the abstract) that these shocks occur in the circumstellar discs. 

Minor comments:

- 2nd para of introduction, define "sufficiently warm and viscous", e.g Ragusa+2016 suggest H/R >~ 0.1 required for this to be true.

RESPONSE: We defined that sufficiently warm discs and added the citation Ragusa+2016.

- third para, HD142527 is a better example, with misalignment between the outer disc and the binary orbit, and between the circum-primary disc and the outer disc (e.g. Marino+2015)

RESPONSE: We have included a sentence describing the misalignment in the HD 142527 system and included two references. 

- second para on page 2 "highly misaligned" should be defined, or remove the word "highly". Similarly please define "sufficiently low disk aspect ratio".

RESPONSE: We have used the term "sufficiently" misaligned and discuss the value of the minimum angle. We mention an estimate of the maximum disc aspect ratio.

- third para on page 2, delete weasel word "somewhat", and "quite" on page 3. Somewhat also appears in two places on page 4.

RESPONSE: We have removed the words "somewhat" and "quite" that appear throughout the letter.

- "variations of accretion"->"accretion variability"

RESPONSE: We have corrected this sentence. 

- section 2 "Smooth" should be "Smoothed" in "Smoothed Particle Hydrodynamics", similarly at the end of section 2.1. Example reference list here includes only papers co-authored by the group, which is OK but comes across as a little self-serving.

RESPONSE: We have corrected the working of "Smoothed Particle Hydrodynamics" and we have added more citations that are not co-authored by our group. 

- discussion of sink particles in section 2.1 should reference original papers where the criteria are described in detail (e.g. Bate et al. 1995). Also should clarify the difference between the "soft" and "hard" accretion boundary employed. That is, is 0.05a the hard boundary (unconditional accretion) or the soft boundary (conditional accretion)?

RESPONSE: We have added the citation of Bate et al. 1995 when discussing the set up of the sink particles and explained our boundary.

- section 2.2, It looks in Figure 2 like the amplitude of the oscillations does decrease slowly with time. There should be some comment on this in the results section, e.g. is this due to depletion of the outer disc? Why did the authors choose to stop at 46 Porb? Is there a numerical limitation caused by the extent of the outer disc?

RESPONSE: The decrease in the amplitude of the oscillations is due to the depletion of the circumbinary disc. After 45 Porb, the circumbinary disc has lost ~40\% of its mass, which is why we did not continue the simulation beyond this time.  

- section 2.2 "that are bound to each binary component", define how this is determined (e.g. presumably just kinetic + potential energy, so neglecting thermal energy?)

RESPONSE: A particle is considered bound to a component when its kinetic + potential energy is negative, neglecting the thermal energy. We have added this in the text. 

- section 2.2 "repeating"->"repeated"

RESPONSE: We are corrected this typo. 

- section 2.2 "after a short initial time", define this in terms of t/Porb

RESPONSE: We have defined this in terms of t/Porb, which is roughly 2 Porb. 

- discussion "very sensitive to the binary"->"sensitive to the binary"

RESPONSE: We have corrected this typo.

- It would be useful for the authors to add a sentence or two outlining what they expect to be different in unequal mass binaries, as are likely, e.g., in most large-cavity transition discs.

RESPONSE: We have added a some sentences in the discussion highlighting the expected results for an unequal mass binary. We expected that the results will be qualitatively the same to the results presented in this letter.  The gas accretion will not be the same for the two discs and their oscillation properties will differ.
